Efficient Checking of Temporal Compliance Rules Over Business Process Event Logs

Verifying temporal compliance rules, such as a rule stating that an inquiry must be answered within a time limit, is a recurrent operation in the realm of business process compliance. In this setting, a typical use case is one where a manager seeks to retrieve all cases where a temporal rule is violated, given an event log recording the execution of a process over a time period. Existing approaches for checking temporal rules require a full scan of the log. Such approaches are unsuitable for interactive use when the log is large and the set of compliance rules is evolving. This paper proposes an approach to evaluate temporal compliance rules in sublinear time by pre-computing a data structure that summarizes the temporal relations between activities in a log. The approach caters for a wide range of temporal compliance patterns and supports incremental updates. Our evaluation on twenty real-life logs shows that our data structure allows for real-time checking of a large set of compliance rules.

==> tex/querying-algo.tex <==

\begin{algorithm}[H]
{\scriptsize{
	\Input{Map $\cIDs$; Map $\aIDs$; Map $\obs$; Map $\deltas$;}
	\Input{String $A$; String $B$; String $q$; Integer $\delta$\;}
	\Output{Set $C$\;}
	\BlankLine

	\textbf{Integer} $a \leftarrow \aIDs(A)$\;
	\textbf{Integer} $b \leftarrow \aIDs(B)$\;
	\textbf{Set} $C \leftarrow \emptyset$\;
	\textbf{List} $X$\;
	\textbf{Map} $S$\; 
	\textbf{Red-Black Tree} $\Pi$\;
	\BlankLine
	
        \If{ $q = \mathit{MAX}$ }{
            $\Pi \leftarrow \deltas((a, b))$\;
            $X \leftarrow$ getTail($\Pi$, ($\delta$, $0$))\;
            \For{ $(\Delta t, c)$ \emph{in} $X$ }{
                \textbf{add} $\cIDs(c)$ \textbf{to} $C$\;
            }
    	}
    	
    	\If{ $q = \mathit{MAXS}$ }{
            $\Pi \leftarrow \deltas((0, b))$\;
            $X \leftarrow$ getTail($\Pi$, ($\delta$, $0$))\;
            \For{ $(\Delta t, c)$ \emph{in} $X$ }{
                \If{$c \notin \obs(a)$}{ 
                    \textbf{add} $\cIDs(c)$ \textbf{to} $C$\;
                }
            }
    	}
    	
    	\If{ $q = \mathit{MAXP}$}{
            $\Pi \leftarrow \deltas((a, b))$\;
            $X \leftarrow$ getTail($\Pi$, ($\delta$, $0$))\;
            \For{ $(\Delta t, c)$ in $X$ }{
                \textbf{add} $\cIDs(c)$ \textbf{to} $C$\;
            }
            
            $\Pi \leftarrow \deltas((0, a))$\;
            $X \leftarrow$ getTail($\Pi$, ($-\infty$, $0$))\;
            
            \For{ $(\Delta t, c)$ in $X$ }{
                \If{$S(c) = \mathit{NULL}$}{\textbf{add} $(c, \Delta t)$ \textbf{to} $S$\;}
            }
            
            $\Pi \leftarrow \deltas((0, b))$\;
            $X \leftarrow$ getTail($\Pi$, ($-\infty$, $0$))\;
            
            \For{ $(\Delta t, c)$ in $X$ }{
                \If{$S(c) = \mathit{NULL} \vee S(c) \geq \Delta t $}{\textbf{add} $\cIDs(c)$ \textbf{to} $C$\;}
            }
    	}
	\BlankLine
    \Return $C$\;
	\caption{\small{Query Data Structure} \\\scriptsize{(example for MAX, MAXS, and MAXP queries)}}\label{alg:querying}
	}}
\end{algorithm}

==> tex/reading-algo2.tex <==
\begin{algorithm}
{\scriptsize{
	\Input{Event Log $\elog$; Time Granularity $\phi$;}
	\BlankLine
	
	\textbf{Integer} $\cc \leftarrow 1$\;%\tcp*{case ID counter} 
	\textbf{Integer} $\ac \leftarrow 1$\;%\tcp*{activity ID counter} 
	\textbf{Map} $\cIDs$ $\leftarrow \emptyset$\;%\tcp*{Key: case label; Value: case ID}
	\textbf{Map} $\aIDs$ $\leftarrow \emptyset$\;%\tcp*{Key: activity label; Value: activity ID}
	\textbf{Map} $\obs$ $\leftarrow \emptyset$\;%\tcp*{Key: activity ID; Value: set of case IDs}
	\textbf{Map} $\activities \leftarrow \emptyset$\;%\tcp*{Key: case ID; Value: sequence of activity IDs}
	\textbf{Map} $\timestamps \leftarrow \emptyset$\;%\tcp*{Key: case ID; Value: sequence of integer timestamps}
	\textbf{Map} $\deltas \leftarrow \emptyset$\;%\tcp*{Key: pair of activity IDs; Value: list of pairs ($\Delta t$, caseID)}
	
	\BlankLine
	\textbf{Integer} $c$\;
	\textbf{Integer} $a$\;
	\textbf{Integer} $t$\;
	\textbf{List} $A$\;
	\textbf{List} $T$\;
	\BlankLine
	
        \For{ $\event \in \elog$ }{	
            $t \leftarrow $ timestampToInteger($\phi$, $\eventime$)\;
            
            \If{$\neg$ containsKey($\cIDs$, $\eventid$)}{
                \textbf{add} ($\eventid$, $\cc$) \textbf{to} $\cIDs$\; 
                \textbf{add} ($\cc$, $\langle 0 \rangle$) \textbf{to} $\activities$\; 
                \textbf{add} ($\cc$, $\langle t \rangle$) \textbf{to} $\timestamps$\; 
                $\cc \leftarrow \cc + 1$\;
            }
            
            \If{$\neg$ containsKey($\aIDs$, $\eventa$)}{
                \textbf{add} ($\eventa$, $\ac$) \textbf{to} $\aIDs$\; 
                \textbf{add} ($\ac$, $\emptyset$) \textbf{to} $\obs$\; 
                $\ac \leftarrow \ac + 1$\;
            } 
            
            $c \leftarrow \cIDs(\eventid)$\;
            $a \leftarrow \aIDs(\eventa)$\;
            $A \leftarrow \activities(c)$\;
            $T \leftarrow \timestamps(c)$\;
            
            \For{$k \in \left[1, \left| A \right| \right]$ }{
                \If{$\neg$ containsKey($\deltas$, ($A_k$, $a$))}{
                    \textbf{add} (($A_k$, $a$), $\emptyset$) \textbf{to} $\deltas$\;
                } 
                \textbf{add} ($t - T_k$, $c$) \textbf{to} $\deltas((A_k, a))$\;
            }
            \textbf{add} $c$ \textbf{to} $\obs(a)$\; 
            \textbf{add} $a$ \textbf{to} $\activities(c)$\;
            \textbf{add} $t$ \textbf{to} $\timestamps(c)$\;
    	}
	\caption{\small{Generate Data Structure} }\label{alg:readlog}
	}}
\end{algorithm}

